Mixing Times of Markov Chains on Degree Constrained Orientations of Planar Graphs

We study Markov chains for $\alpha$-orientations of plane graphs, these are orientations where the outdegree of each vertex is prescribed by the value of a given function $\alpha$. The set of $\alpha$-orientations of a plane graph has a natural distributive lattice structure. The moves of the up-down Markov chain on this distributive lattice corresponds to reversals of directed facial cycles in the $\alpha$-orientation. We have a positive and several negative results regarding the mixing time of such Markov chains. A 2-orientation of a plane quadrangulation is an orientation where every inner vertex has outdegree 2. We show that there is a class of plane quadrangulations such that the up-down Markov chain on the 2-orientations of these quadrangulations is slowly mixing. On the other hand the chain is rapidly mixing on 2-orientations of quadrangulations with maximum degree at most 4. Regarding examples for slow mixing we also revisit the case of 3-orientations of triangulations which has been studied before by Miracle et al.. Our examples for slow mixing are simpler and have a smaller maximum degree, Finally we present the first example of a function $\alpha$ and a class of plane triangulations of constant maximum degree such that the up-down Markov chain on the $\alpha$-orientations of these graphs is slowly mixing.

==> updfig <==
#! /bin/csh -f

cd Figures

fig2dev -L pdftex $1.fig > $1.pdf
fig2dev -L pstex $1.fig > $1.eps

fig2dev -L pstex_t -p $1.pstex $1.fig > $1.pstex_t

perl -p -i.bak -e 's#.pstex##g' $1.pstex_t

perl -p -i.bak -e 's#\\begingroup#\n\\multiply\\unitlength by \\magproz\n\\divide\\unitlength by 100\n\n\\begingroup#g' $1.pstex_t

perl -p -i.bak -e 's#\includegraphics{#\includegraphics[scale=\\figscale]{#g' $1.pstex_t

rm $1.pstex_t.bak

cd ..

##############################
# new version of UPDPSF 
# renamed to UPDFIG
# new feature, generates pdf and eps and doesn't specify
# which to include. So everything can be used with
# latex and pdflatex without any change.

